Improving Compositional Generalization Using Iterated Learning and Simplicial Embeddings

Compositional generalization, the ability of an agent to generalize to unseen combinations of latent factors, is easy for humans but hard for deep neural networks. A line of research in cognitive science has hypothesized a process, ``iterated learning,'' to help explain how human language developed this ability; the theory rests on simultaneous pressures towards compressibility (when an ignorant agent learns from an informed one) and expressivity (when it uses the representation for downstream tasks). Inspired by this process, we propose to improve the compositional generalization of deep networks by using iterated learning on models with simplicial embeddings, which can approximately discretize representations. This approach is further motivated by an analysis of compositionality based on Kolmogorov complexity. We show that this combination of changes improves compositional generalization over other approaches, demonstrating these improvements both on vision tasks with well-understood latent factors and on real molecular graph prediction tasks where the latent structure is unknown.

==> section_app1.tex <==
\begin{algorithm}[tb]
\caption{Proposed SEM-IL algorithm}
    \begin{algorithmic}
        \STATE Split the network into $h(\vx)$ and $g(\vz)$, then add an SEM bottleneck to discretize $\vz$
        \FOR{$\mathit{t}=0$ {\bfseries to} $T_\mathit{gen}$}
            % \STATE \textit{\# Initialization Phase}
            \STATE Initialize the student speaker $h^S_t(\vx)$
            \STATE \textit{\# \qquad Imitation Phase (start from the second generation)}
            \IF{$t > 0$}
                %\STATE Initialize the student by copying the teacher in the previous generation: $h^S_t\leftarrow h^T_{t-1}$
                    \FOR{$i=0$ {\bfseries to} $I_{imit}$}
                    \STATE Sample a batch $\vx$ from the training set $\mathcal{D}_{train}$
                    \STATE Sample the pseudo labels from teacher's prediction (one-hot vectors) $\vg_{1:L}\sim h_t^T(\vx)$
                    \STATE Calculate the student's prediction $\vz=[\hat{z}_1,...,\hat{z}_L]=h_t^S(\vx)$ 
                    \STATE Update $h_t^S(\cdot)$ with multi-label cross-entropy loss $\mathcal{L}_{ml}=\sum_{i=1}^L \vg_i^\top\cdot\log \hat{z}_i$ 
                \ENDFOR
            \ENDIF              
            \STATE \textit{\# \qquad Interaction Phase (regular training on the downstream task)}
            \FOR{$i=0$ {\bfseries to} $I_{int}$}
                \STATE Initialize the listener $g_t(\vz)$ randomly
                \STATE Sample a batch $(\vx,\vy)$ from the training set $\mathcal{D}_{train}$
                \STATE Calculate the downstream prediction $\hat{\vy}=(g_t\circ h^S_t)(\vx)$
                \STATE Update the parameters of $h^S_t$ and $g_t$ to minimize the downstream loss $\mathcal{L}_{ds}(\hat{\vy},\vy)$
            \ENDFOR
            \STATE The student becomes the teacher for the next generation: $h_{t+1}^T\leftarrow h_{t}^S$
        \ENDFOR
        \STATE Return the last (or the best) $(g_t\circ h_t^S)(\vx)$ for the downstream task
    \end{algorithmic}
    \label{alg:il}
\end{algorithm}

\section{The Ladder of Systematicity}
\label{sec:app_ladder_of_representation}

\begin{table}[t]
    \caption{What information contained in $\vz$ on the ladder and their corresponding capabilities.
             $H(\cdot)$ is the entropy, $\leftrightarrow$ means bijection, $\Leftrightarrow$ means isomorphism bijection.}
    \vskip 0.1in
    \centering\begin{tabular}{cccccc}
    \hline
               & Infor. in $\vz$ & Train acc.   & ID-gen       & \begin{tabular}[c]{@{}c@{}}OOD-gen with\\ seen concepts\end{tabular} & Sys-gen      \\ \hline
    \rowcolor[HTML]{EFEFEF} 
    Stage I   & $H(\vG\mid\vz)>0$                                                                    & $\times$     & $\times$     & $\times$                                                             & $\times$     \\
    Stage II  & \begin{tabular}[c]{@{}c@{}}$H(\vG\mid\vz)=0$\\ $H(\vz\mid\vG)>0$\end{tabular} & $\checkmark$ & $\checkmark$ & $\times$                                                             & $\times$     \\
    \rowcolor[HTML]{EFEFEF} 
    Stage III & $\vz\leftrightarrow\vG$                                                                     & $\checkmark$ & $\checkmark$ & $\checkmark$                                                         & $\times$     \\
    Stage IV  & $\vz\Leftrightarrow\vG$                                                                     & $\checkmark$ & $\checkmark$ & $\checkmark$                                                         & $\checkmark$ \\ \hline
    \end{tabular}
    \label{tab:ladders}
\end{table}

To figure out what $\vz$ we need in order to generalize well systematically,
we propose the ``ladder of systematicity'' in Figure~\ref{fig:datagen_ladder}.
To justify our claims, 
this appendix will discuss how we could climb the ladder step by step by analyzing how the corresponding requirements are generated.
A formal version of Hypothesis~\ref{prop:z_sysgen},
which is necessary for reaching the final stage of the ladder,
is also provided.
In short,
we find only relying on the mutual information between $\vz$ and $\vG$ cannot reach the final rung of the ladder:
we need other inductive biases, which is the main motivation of this paper.

\subsection{Stage I: z misses some important information in G}
%\textbf{$\bullet$\quad Stage I: $\vz$ misses some important information in $\vG$}

The learned representation would have $H(\vG\mid\vz)>0$ at this stage.
As $Y=\mathsf{GenY}(\vG,\epsilon)$ and $\hat{Y}=g(\vz)$ are assumed to be invertible (here $Y$ and $\hat{Y}$ are random variables),
this condition can be rewritten as $I(Y;\hat{Y})<H(Y)$
\footnote{Using the fact that $H(\vG\mid\vz)=H(Y\mid\hat{Y})=H(Y) - I(Y;\hat{Y})$.}.
Hence following the analysis in \cite{shwartz2017opening},
a model with such an encoder $\vz=h(\vx)$ even cannot achieve high enough training performance,
let alone generalizing to unseen test distributions.
This condition might occur when the model underfits the training data, 
e.g., at the beginning of training or the model's capacity is too small.
To make an improvement,
one can increase the model size or train longer.

\subsection{Stage II: z not only contains all information in G but also some from O}
%\textbf{$\bullet$\quad Stage II: $\vz$ learns all information in $\vG$, but also some from $\vO$}

At this stage,
the learned representation would have $H(\vG\mid\vz)=0$ and $H(\vz\mid\vG)>0$.
This means $h(\vx)$ remembers additional information that $\vG$ doesn't have,
e.g., noisy information in $\vO$.
As $I(Y;\hat{Y})=H(Y)$,
the model would have perfect training performance and could also be able to generalize well when training and test datasets share the same distribution.
However, when facing the out-of-distribution generalization problem,
especially when a spurious correlation exists between some factors in $\vO$ and $\vG$,
the extra information learned by $\vz$ can mess the predictions up.
Such a phenomenon is named ``short-cut learning'' and is quite common in many deep-learning systems \cite{geirhos2020shortcut}.
For example, if the background strongly correlates with the object in the training set 
(e.g., a cow usually co-occurs with the grass while a seagull usually co-occurs with the beach),
the DNN then tends to rely more on these ``short-cut'' features (e.g., the background rather than the object) during training.
If such correlations disappear or reverse in the test set,
the models relying on factors in $\vO$ cannot generalize well to a new distribution.

%\textbf{$\bullet$\quad Making improvement: loss based on information-bottleneck}
\paragraph{Making improvement -- loss based on information-bottleneck}
To make an improvement,
the model should eliminate the task-irrelevant information as much as possible.
Based on this principle,
authors of \cite{tishby2000information} propose to minimize the following information bottleneck equations:
\begin{equation}
    \max \quad I(Z;Y)-\beta I(Z;X), \quad \beta>0,
\end{equation}
which means the learned $\vz$ should extract as much as information from $Y$ (or equivalently, $\vG$) and forget as much as irrelevant information about $X$ (i.e., those in $\vO$).
This method is also widely applied in other relevant tasks,
like domain adaptation \cite{li2022invariant},
invariant risk minimization \cite{ahuja2021invariance}, and etc.

%\textbf{$\bullet$\quad Making improvement: data augmentation}
\paragraph{Making improvement -- data augmentation}
Another simple and efficient way to make improvements is data augmentation:
one can assume some task-irrelevant factors in $\vO$ and design specific data augmentation methods to teach the model to be insensitive to them.
For example, if we believe that the label of an image should be irrelevant to color jittering, random cropping, rotation, flipping, etc.,
we can apply random augmentations during training and treat the differently augmented $\vx$ and $\vx'$ as the same class.
Then the model would inherently learn to be insensitive to such factors and hence forget the corresponding information.
One interesting thing about data augmentation is that it can be designed and applied in a reverse direction,
i.e., we can break some semantic factors and train the model to be insensitive to the broken samples.
For example, believing the shape of the image and order of the words are semantic factors in $\vG$,
the authors of \cite{puli2022nuisances} propose to randomly rotate the image patches or words to make negative samples.
Those models that perform well on these negative samples are more likely to rely on the factors in $\vO$.

%\textbf{$\bullet$\quad Making improvement: auxiliary task design, e.g., SSL}
\paragraph{Making improvement -- auxiliary task design, e.g., SSL}

Furthermore,
one can also consider designing auxiliary tasks in addition to the downstream task,
e.g., pretrain using self-supervised learning (SSL) and finetune on the target task.
In \cite{shi2022robust},
the authors empirically show that the representations learned via SSL usually generalize better than those learned via supervised learning when facing OOD downstream problems,
even when the models are trained using a similar amount of data samples.
There are also some works demonstrating that SSL representations encode more semantic information about the input image \cite{caron2021emerging},
which is a sign that auxiliary tasks like SSL can introduce extra biases that favor information in $\vG$.

Consider the first group of SSL methods,
which are usually based on contrastive loss,
e.g., SimCLR \cite{chen2020simple}, MoCo \cite{he2020momentum}, etc.
These methods usually require $h(\vx_i)$ and $h(\vx'_i)$ to be similar while $h(\vx_i)$ and $h(\vx_j), i\neq j$ to be distinct,
where $\vx_i$ is the anchor input,
$\vx_i'$ is the augmentation of it,
and $\vx_j$ is another different image.
The carefully designed augmentation can encourage the model to ignore some task-irrelevant factors that belong to $\vO$.
Imagine $\vx_i'$ is generated by deleting the background of $\vx_i$.
As the training enforces $d_z(h(\vx), h(\vx'))$ to be small,
the learned model will then become insensitive to the information in the background,
and hence avoid relying on this ``short-cut'' feature.
Note that the contrastive SSL is utilizing the bias from data augmentation in a more aggressive way:
the SSL algorithm will tell the model that $\vx$ and $\vx'$ are the \textit{same image} 
while the supervised learning only inform the model that $\vx$ and $\vx'$ belong to the \textit{same class}. 

Another line of SSL is built on reconstruction tasks,
like denoising auto-encoder (DAE \cite{vincent2008extracting}) and masked auto-encoder (MAE \cite{he2022masked}).
The $h(\vx)$ in these methods is usually trained in an auto-encoder fashion:
using a reconstruction network $r(\vz):\mathscr{Z}\rightarrow \mathscr{X}$,
we require the reconstructed $\vx_{recon}=(r\circ h)(\vx)$ to be similar to the original input $\vx$.
As the above equation has a trivial solution,
i.e., $(r\circ h)(\cdot)=identity$,
which means $h(\vx)$ copies every details about $\vx$ (including all $\vO$ and $\vG$),
some early works like denoising auto-encoder \cite{vincent2008extracting} propose to add noise on $\vx$ to encourage non-trivial solutions.
Depending on the noise we introduce,
the model will learn to ignore different factors accordingly,
which seems quite similar to the data augmentation mentioned in contrastive SSL methods.
To encourage $h(\vx)$ to extract more useful semantic information in $\vG$,
methods like MAE \cite{he2022masked} propose to mask most of the patches of the input image and try to make reconstructions based on the remaining patches.
Such methods exhibit amazing reconstruction performance (not in terms of high resolution, but the precise semantic reconstruction),
which also implies that the $h(\vx)$ trained in this way is capable of extracting high-level semantic generating factors (those are likely in $\vG$).
Furthermore,
methods like BEiT \cite{bao2022beit} and iBOT \cite{zhou2022image} also patchify and mask the input images,
and concurrently, impose extra constraints on $\vz$ by comparing them with the descriptions generated by the big language model.
Such designs also encourages $h(\vx)$ to extract high-level semantic information,
as illustrated in \cite{caron2021emerging}.

In summary,
as the SSL algorithms learn good $\vz$ by designing loss or tasks on it,
we can introduce extra inductive bias via auxiliary tasks.
By requiring $\vz$ to be invariant when adding noise or conducting data augmentation on $\vx$,
the task-irrelevant information can be ruled out during learning.
By requiring $\vz$ contains the necessary information for reconstruction when only part of $\vx$ is observable,
the task-relevant semantic information can be strengthened during learning.
By combining these principles,
it is possible for us to learn good $h(\vx)$ that only extracts information in $\vG$.
With the help of these methods,
our $\vz$ might learn \textit{exactly} all information in $\vG$,
which means the third rung is achieved.


\subsection{Stage III: z learns exactly all information in G, i.e., \texorpdfstring{$h(\cdot)$}{h(.)} leads to a bijection}
%\textbf{$\bullet$\quad Stage III: $\vz$ learns exactly all information in $\vG$, i.e., $f$ leads to a bijection}

Starting from Stage II, 
if we can design clever training methods (e.g., adding regularization, data augmentation, auxiliary task, etc.) and make our $h(\vx)$ to be insensitive to some $\vO$,
ideally,
we can learn an almost perfect encoder that extracts exactly all information contained in $\vG$.
In this case,
we have $H(\vG\mid\vz)=0$ and $H(\vz\mid\vG)=0$,
i.e., $h(\cdot)$ leads to a bijection between $\vz$-space and $\vG$-space,
which is denoted as $\vz\leftrightarrow\vG$.
Ideally,
such $\vz$ can generalize well even when $P_{train}\neq P_{test}$,
as long as all the concepts in the test set are seen by $h(\vx)$ during training,
i.e., $\mathsf{supp}[P_{test}(\vG)]\subseteq\mathsf{supp}[P_{train}(\vG)]$.
However, we speculate that even $h(\vx)$ on Stage III will struggle in the sys-gen problem,
as the problem assumes $\mathsf{supp}[P_{test}(\vG)]\cap\mathsf{supp}[P_{train}(\vG)]=\emptyset$.
In other words,
we need the model to decompose and recombine the learned concepts in a similar way to the ground-truth-generating mechanism.
To achieve this goal, we need Stage IV.

\subsection{Stage IV: \texorpdfstring{$h(\cdot)$}{h(.)} leads to a isomorphism bijection between z and G}
\label{sec:app_ladder_of_representation_stage4}
%\textbf{$\bullet$\quad Stage IV: $f$ leads to a distance-preserving bijection between $\vz$ and $\vG$}

To generalize well systematically,
we not only need $\vz$ contains exactly all information in $\vG$,
the structure of $\vG$ should also be embodied in $\vz$,
which means $h(\cdot)$ should lead to a isomorphism bijection between $\vz$-space and $\vG$-space (i.e., $\vz\Leftrightarrow\vG$).
Specifically,
we need the learned $\vz$ to satisfy the following (it is easy to verify that such $\vz$ satisfies the linear disentanglement requirement mentioned in \cite{higgins2018towards}, if factors in $\vG$ are assumed to be independent):

\begin{tcolorbox}[title=Detailed definition of Hypothesis~\ref{prop:z_sysgen}]
To generalize well systematically, we need $\vz\Leftrightarrow\vG$,
which requires:
\begin{enumerate}\label{prop:z_sysgen_formal}
    \item $\vz\leftrightarrow\vG$, i.e., $h(\cdot)$ leads to a bijection between $\vz$ and $\vG$;
    \item $P(\vz)$ and $P(\vG)$ factorize in a similar way;
    \item Each $z_i$ maps to some $G_{\vw_i}$, where $\vw$ is a permutation vector of length $L$, such a mapping is invariant\footnote{For example, $z_1$ always encode color and $z_2$ always encode shape.};
    \item For each $z_i$, the mapping between $z_i=k$ and $G_{\vw_i}=\vu_k$ is invariant\footnote{For example, $z_1=0$ always means blue and $z_1=1$ always means red.}, where $\vu$ is a permutation vector of length $V_{\vw_i}$.
\end{enumerate}
\end{tcolorbox}

\begin{figure}[ht]
    \begin{center}
    \centerline{\includegraphics[width=0.8\columnwidth,trim=0 0 0 0, clip]{figures/systematic_mapping.pdf}}
    \caption{A systematic mapping and a holistic mapping.
             Although holistic mapping seems to have fewer ``crossings'', its topological similarity is lower than the systematic one.}
    \label{fig:sys_mapping}
    \end{center}
\vskip -0.2in
\end{figure}

We call such mappings \textbf{systematic} and call the other bijections \textbf{holistic}.
To better understand the difference between these two types of mappings,
we consider a simple example where the generating factors are $\vG=[G_1, G_2]$, $G_1=\{\text{blue, red}\}$ and $G_2=\{\text{circle, box}\}$,
and the representations are $\vz=[z_1,z_2]$, $z_1=\{0,1\}$ and $z_2=\{0,1\}$.
Hence the space of $\vG$ is $\{$ blue circle, blue box, red circle, red box $\}$,
and the space of $\vz$ is $\{00,01,10,11\}$.
To generate a systematic mapping,
we can first decide the meaning of $z_i$,
e.g., $z_1$ represents the shape and $z_2$ represents the color.
After that,
we assign vocabularies in $z_i$ to denote different meanings,
e.g., $z_1=0\rightarrow \text{circle}$, $z_1=1\rightarrow \text{box}$, $z_2=0\rightarrow \text{blue}$, and $z_2=1\rightarrow \text{red}$.
Combining these two steps,
we generate a systematic mapping, as illustrated in Figure~\ref{fig:sys_mapping}(a).
Any bijections that cannot be decomposed in this way are holistic mappings, like Figure~\ref{fig:sys_mapping}(b).
Obviously,
the systematic mappings can generalize systematically while the holistic ones cannot.
However, finding a systematic mapping from all possible bijections is a hard problem,
as the number of systematic mappings is much smaller than the holistic ones:
assuming we have $L=3$ different $G_i$ and each with $V=3$ possible values,
there are roughly $10^{3}$ systematic mappings ($L!\cdot(V!)^L$),
and $10^{28}$ holistic mappings ($(V^L)!-L!\cdot(V!)^L$).

Another important characteristic of systematic mappings is the ``distance-preserving'' ability.
In other words,
they will map two $\vx$ with similar $\vG$ to two similar $\vz$ in the representation space,
i.e., $\vz$ preserve the topological structure of $\vG$.
We can use topological similarity ($\rho$, defined in Equation~\ref{eq:topsim}) to quantify how systematic a mapping is.
Usually,
for all bijections,
mappings with larger $\rho$ are more systematic.
To sum up the aforementioned four stages of the learned $\vz$, 
we list the conditions that $\vz$ must satisfy and their capabilities in Table~\ref{tab:ladders}.

\subsection{Relationship with disentangled representations}
\label{sec:app_ladder_of_representation_relation_to_disentangle}

Readers might notice that our problem settings and the requirements for $\vz$ mentioned in Hypothesis~\ref{prop:z_sysgen} are quite similar to those discussed in disentanglement representation learning \cite{higgins2018towards}.
Here we explain the connections and differences between them.

%\textbf{$\bullet$\quad We care more on downstream tasks:}
\paragraph{We care more about downstream tasks.}
In disentanglement representation learning,
people focus more on a general property of the learned representation by assuming the existence of independent semantic generating factors.
Disentanglement is then considered a desired property of such representations.
Works in this line try to formalize this property and believe this property is beneficial for multiple downstream tasks.
However, as the downstream task is not incorporated in such analysis,
it is hard to conclude whether specific factors are semantic or not (remember the split of $\vO$ and $\vG$ highly depends on the task).
On the other hand, this paper focuses more on the generalization ability of the learned representations on specific downstream task(s).
We directly optimize the loss of the downstream task in the interaction phase,
which we believe can regularize the representations more efficiently.

%\textbf{$\bullet$\quad We don't strictly require a disentangled $\vz$:}
\paragraph{We don't strictly require a disentangled $\vz$.}
Although representations with properties like consistency or restrictiveness mentioned in \cite{Shu2020Weakly} could be beneficial for the downstream tasks,
it seems not necessary to have all of them.
In other words,
disentanglement is a sufficient but not necessary requirement for a model to generalize well in downstream tasks.
That is because the factorization of $\vG$ could be non-trivial (as nature is not simple).
We believe that capturing the hidden structure of $\vG$ and $\mathsf{GenY}(\cdot)$ using $\vz$ and $g(\cdot)$ is more important than mapping an involved generating mechanism to a disentangled system.
Additionally, implicitly splitting $\vO$ from $\vG$ is rather crucial in our settings,
which is rarely discussed in the fields of disentanglement representation learning.

%\textbf{$\bullet$\quad We rely on the discreteness of the factors:}
\paragraph{We consider discrete factors.}
This might be a shortcoming of our current analysis.
Being inspired by how human language evolves,
it is natural to start from the discrete factors and representations.
Our experimental results also benefit a lot from the discreteness,
e.g., using cross-entropy loss to amplify the learning speed advantage,
sampling pseudo labels to strengthen the inductive bias, etc.
However, as nature might not be purely discrete,
incorporating the continuous latent space is crucial to enlarge the scope of our study.
We would leave this in our future work.






==> section_app2.tex <==
\section{Iterated Learning and Why it Works}
\label{sec:app_il_examples}

Reaching the final rung is not easy for deep neural networks,
because most of the common loss and training designs focus on information-related targets.
As systematic and holistic mappings are all bijections,
information-related metrics cannot separate them apart.
Fortunately, as mentioned in Section~\ref{sec:intro},
a civilized human can solve sys-gen problems with relative ease,
and human languages are perfect examples of systematic mappings \cite{hockett1960origin}.
To explain how humans gain such an ability,
researchers in cognitive science and evolutionary linguistics propose many interesting hypotheses.
Iterated learning (IL, \cite{kirby2008cumulative}) discussed in this work is one of them.

To provide a panorama of iterated learning and its applications in different fields,
this appendix will first give an intuitive explanation using some lab experimental results.
Then, experiments on Bayesian agents are introduced to explain why the posterior of systematic mappings gradually dominates.
As the bias for highly systematic mappings is the crux of iterated learning 
(it is assumed to be inborn within the human cognitive system),
we will also discuss how such a preference is embodied in deep learning systems.


\subsection{Iterated Learning in Lab Experiments using Lewis Language Game}

\begin{algorithm}[t]
\caption{A typical IL algorithm used in lab experiments}
\label{alg:app_il}
    \begin{algorithmic}
        \STATE Prepare input images and available vocabulary
        \FOR{$\mathit{t}=0$ {\bfseries to} $T_\mathit{gen}$}
            % \STATE \textit{\# Initialization Phase}
            \STATE Select two people from all candidates, call them Alice[t] and Bob[t]
            \STATE \textit{\# \qquad Imitation Phase}
            \IF{$t > 0$}
                \STATE Alice[t] learns from the dataset $\mathcal{D}_{t-1}$
            \ENDIF
            \STATE \textit{\# \qquad Interaction Phase}
            \FOR{$i=0$ {\bfseries to} $I_{int}$}
                \STATE [Can be other tasks requiring unambiguous language from Alice.]
                \STATE Alice[t] play the Lewis Language Game with Bob[t]
                \STATE Alice[t] and Bob[t] switch the role and play the game again
            \ENDFOR
            \STATE \textit{\# \qquad Transmission Phase}
            \STATE Alice[t] generate the dataset $\mathcal{D}_{t}$ 
        \ENDFOR
        \STATE Return how Alice[$T_{gen}$] name all the images in the dataset.
    \end{algorithmic}
\end{algorithm}

\begin{figure}[t]
\vskip -0.2 in
    \begin{center}
    \centerline{\includegraphics[width=\textwidth]{figures/iterated_learning.pdf}}
    \caption{The lab experiments conducted in \cite{kirby2015compression}.}
    \label{fig:app_iterated_learning}
    \end{center}
\vskip -0.3in
\end{figure}

%\textbf{$\bullet$\quad Lab experiment using Lewis language game}
%\paragraph{Lab experiments using Lewis language game}
As denoted in \cite{kirby2008cumulative},
iterated learning is a process where one individual learns by observing the output of another individual, who learned in the same way.
In this multiple-generation learning procedure,
the shared language among learning agents will gradually become more systematic under the compressibility pressure (imposed during imitation) and expressivity pressure (imposed during interaction).
To simulate this process,
authors of \cite{kirby2015compression} design a two-phases learning procedure illustrated in Algorithm~\ref{alg:app_il} and Figure~\ref{fig:app_iterated_learning}.
In the interaction phase,
the speaker (Alice) and listener (Bob) must cooperate to accomplish a Leiws referential game (see the left panel in Figure~\ref{fig:app_iterated_learning}).
Specifically,
Alice will first create a name for the given objects and talk that to Bob.
After receiving this message, Bob needs to select the correct object shown to Alice among some candidates.
If correct, both of them are rewarded. This phase terminates when they can achieve a high enough success rate.
To succeed in this game,
the shared language should be expressive enough to avoid any ambiguities --
we expect the language to be a bijection.
Then, we select another new naive candidate (Alice[t+1]) and let it learn the naming system created by Alice[t] and Bob[t].
In this phase,
those highly structural mappings should be easier for a human to remember,
which is how the compressibility pressure is imposed.
After that, Alice[t+1] will play the same game with another Bob[t+1] and the interaction phase starts again.
We provide the languages generated by Alice[0] and Alice[10] in the right panel in Figure~\ref{fig:app_iterated_learning}:
it is clear that an interesting structure emerges in the language generated by Alice[10].
There are also plenty of similar lab experiments that support the ``two pressures'' and cultural evolution hypothesis using IL-like training methods,
e.g., \cite{fay2010interactive, ferdinand2019cognitive, motamedi2022improvisation, motamedi2019evolving}.
Although these methods have different types of input, game designs, learning procedures, vocabularies (like gesture language), etc.,
the conclusion of them is quite consistent:
compressibility and expressivity pressures are crucial for the emergence of systematical mappings,
which inspires us a lot.

\subsection{Iterated Learning for Bayesian Agents}
%\textbf{$\bullet$\quad Bayesian agent analysis -- toy dataset}

To verify that the emergence of systematic mappings in iterated learning is not an accident,
authors of \cite{beppu2009iterated, 3dshapes18} provide a guarantee by analyzing the behavior of Bayesian agents.
Consider the toy example mentioned in Appendix~\ref{sec:app_ladder_of_representation_stage4},
where the space of $\vG$ is $\{$ blue circle, blue box, red circle, red box $\}$,
and that of $\vz$ is $\{00,01,10,11\}$.
We use $l\in\mathscr{L}$ to denote a mapping between $\vz$ and $\vG$,
where $\mathscr{L}$ denotes the space of all possible mappings.
In this toy example,
we have 256 different mappings\footnote{This value is calculated as $(V^L)^{(V^L)}$. Here we see the size of all possible mappings is extremely huge when $L$ and $V$ increase, which makes the analysis based on mappings hard to scale.}.
The output of a Bayesian agent is defined as a categorical distribution parameterized by $\mathbb{\theta}$: $P(\vL)=\mathsf{Cat}[\theta_1,...,\theta_{256}]$,
where $\vL$ is the vector form of all possible $l$.
In this analysis,
we \textbf{assume} the prior distribution of a mapping is negatively correlated with its \textit{coding length} $\alpha$,
i.e., $P(l;\alpha)\propto 2^{-\alpha}$ for each $l$.
Usually, the easier-to-learn mappings (i.e., more systematic mappings) have higher prior.
In Table~\ref{tab:app_coding_length},
we demonstrate how to calculate the coding length for the two mappings illustrated in Figure~\ref{fig:sys_mapping}.
Note that the mapping that has the highest prior is a degenerate mapping,
i.e.,  S: \{00, 01, 10, 11\} $\rightarrow$ red box,
where $\alpha=27$ and $P(l)\approx 0.6$.
We also show the topological similarity and the prior probabilities of all 256 possible languages in Figure~\ref{fig:app_topsim_prior}.

\begin{table}[ht]
    \vskip 0in
    \caption{How to calculate the coding length of a mapping, where $\alpha$ is how many characters 
             (including space and unique symbol, e.g., $\rightarrow$ and $:$) are used to express the grammar.}
    \centering\begin{tabular}{ccccccccl}
    \hline
    \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}A systematic mapping\\ $\alpha=43, P(l)\sim 10^{-6}$\end{tabular}} &
       &
      \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}}A holistic mapping\\ $\alpha=56, P(l)\sim 10^{-10}$\end{tabular}} \\ \hline
    S   &   & $\rightarrow$ & z2, z1 &  &    &               &             &  \\
    z2: & 0 & $\rightarrow$ & blue   &  & S: & $\rightarrow$ & blue circle &  \\
    z2: & 1 & $\rightarrow$ & red    &  & S: & $\rightarrow$ & red circle  &  \\
    z1: & 0 & $\rightarrow$ & circle &  & S: & $\rightarrow$ & red box     &  \\
    z1: & 1 & $\rightarrow$ & box    &  & S: & $\rightarrow$ & blue box    &  \\ \cline{1-8}
    \end{tabular}
    \label{tab:app_coding_length}
\end{table}

%\textbf{$\bullet$\quad Bayesian agent analysis -- results}
Recall the iterated learning procedure mentioned in Algorithm~\ref{alg:app_il},
which requires one agent to learn from the $(\vx, \vm)$ pairs generated by another agent.
The message $\vm$ is generated by $\vm=l(\vx)$,
where $l\sim P(\vL | \vx; \text{Alice[t]})$ is a mapping sampled from an agent.
The dataset used for imitation is $\mathscr{D}_t\triangleq(\vx_n,\vm_n)_{n=1}^N$
Under these notations,
we can formulate the iterated learning procedure as the following:
\begin{itemize}
    \item Imitation phase: an initialized agent, i.e., Alice[t+1] with prior $P(\vL;\alpha)$, learns from $\mathscr{D}_t$,
          which is sampled from Alice[t]'s posterior distribution. The agent after learning would have the following posterior:
            \begin{equation}
                P(\vL;\text{Alice[t+1]}) = P(\vL|\mathscr{D}_t)\propto P(\mathscr{D}_t|\vL)\cdot P(\vL;\alpha)\nonumber
            \end{equation}
    \item Interaction phase: Alice[t+1] communicate with Bob[t+1] (directly copy Alice[t+1]'s posterior) to accomplish the task.
          $\mathscr{D}_{comm}$ is sampled from $P(\vL;\text{Alice[t+1]})$,
          but only contains the mappings that the game succeeds. 
          In other words, the following update (for both Alice and Bob) only happens when the game succeeds:
            \begin{equation}
                P(\vL;\text{Alice[t+1]}) = P(\vL|\mathscr{D}_{comm})\propto P(\mathscr{D}_{comm}|\vL)\cdot P(\vL;\text{Alice[t+1]})\nonumber
            \end{equation}
    \item Transmission phase: prepare the data $\mathscr{D}_{t+1}$ for the next generation.
          Note that in the Bayesian example, the learning starts with the imitation phase, where $\mathscr{D}_{0}$ is manually selected from 256 languages.
          We use this setting to show that systematic mappings can gradually dominate whatever $\mathscr{D}_{0}$ we choose.
\end{itemize}

In the above procedure,
the compressibility pressure is embodied in a manually designed prior distribution where more reusable principles lead to a higher probability.
The expressivity pressure is imposed via how $\mathscr{D}_{comm}$ is generated: it only contains the mappings that make the game succeed.
For this toy case,
we can calculate the weighted proportion 
(i.e., the summation of the posteriors) 
of different types of languages and observe how it evolves during iterated learning,
as illustrated in Figure~\ref{fig:app_ratio_language}.
It is clear that the systematic mappings gradually dominate as the learning progress.
For ablation studies,
we can consider a compressibility-only case by removing the game-success requirement when generating $\mathscr{D}_{comm}$,
and an expressivity-only case using a uniform prior $P(l)=1/256$.
The results in Figure~\ref{fig:app_ratio_language} match our assumptions quite well.
Figure~\ref{fig:app_posterior} provides a more detailed observation of how the posterior of all mappings changes during training.
In the first generation, we see the dominant mapping is a holistic one,
which is our $\mathscr{D}_0$. 
Then gradually, under the two pressures, 
the posterior of systematic mappings gradually increases and finally dominates. 

In summary,
the analysis of the Bayesian agents provides a potential direction for a theoretical understanding of why iterated learning works.
However,
analyzing the learning behavior in the mapping space is hard to scale:
the size of all possible mappings grows too fast!
It is also hard to incorporate the bias of model structure and gradient descent into this framework.

\begin{figure}[ht!]
\vskip -0.2in
    \begin{center}
    \centerline{\includegraphics[width=0.85\textwidth, trim={50, 10, 50, 30}, clip]{figures/topsim_prior.pdf}}
    \caption{Topological similarity (defined in Equation~\ref{eq:topsim}) and the prior probability of all 256 different mappings.
            It is clear that the prior of systematic mappings is sandwiched between that of degenerate and holistic mappings.
            That is why we need the expressivity pressure to rule out those degenerate mappings.
            Some mappings in the ``other'' group also have relatively large prior,
            because they contain degenerate components (e.g., mapping two or three objects to the same message).}
    \label{fig:app_topsim_prior}
    \end{center}
\vskip -0.2in
\end{figure}

\begin{figure}[ht!]
\vskip -0.05in
    \begin{center}
    \centerline{\includegraphics[width=0.85\textwidth, trim={0, 0, 0, 0}, clip]{figures/ratio_languages.png}}
    \caption{Ratio of three different types of mappings during iterated learning (curves are the average of 15 different runs, shadow region is the variance).
            Left to right: 1.) $\mathscr{D}_0$ is a holistic mapping;
            2.) $\mathscr{D}_0$ is a degenerate mapping;
            3.) Starting from a holistic $\mathscr{D}_0$, but no longer conduct an interaction phase during training.
                Hence the degenerate language, which has the highest prior, will gradually dominate;
            4.) Ablating the compressibility pressure by using a uniform prior distribution.}
    \label{fig:app_ratio_language}
    \end{center}
\vskip -0.2in
\end{figure}

\begin{figure}[ht!]
\vskip -0.2in
    \begin{center}
    \centerline{\includegraphics[width=0.85\textwidth, trim={50, 50, 50, 50}, clip]{figures/posterior_diff_gen.pdf}}
    \caption{The posterior probabilities of all at the end of different generations.}
    \label{fig:app_posterior}
    \end{center}
\vskip -0.2in
\end{figure}


\subsection{Preference of Systematicness in Deep Learning: Three Hypotheses}
\label{sec:app_il_examples_bias}

Although iterated learning reliably prompts the emergence of systematic mapping in lab experiments and Bayesian agent cases, 
directly applying it to deep learning is not trivial:
as we are not sure whether the preference for systematic mappings still exists for the neural agents. 
Remember in lab experiments, the human's cognition system automatically favors systematicness.
For the Bayesian agents,
the prior probability is manually designed to be inversely correlated to the coding length.
Hence in this subsection,
we will introduce three hypotheses of how the compressibility bias is embodied in deep neural network training.
Specifically,
they are 1.) the learning speed advantage hypothesis;
2.) sample  alignment hypothesis discussed in Section~\ref{sec:toy_experiments};
and 3.) the coding length and active basis hypothesis, which is more theoretical and would be extended in our future work.

%\textbf{$\bullet$\quad The learning speed advantage hypothesis in GD}
\paragraph{The learning speed advantage in GD}

\begin{wrapfigure}{r}{0.5\textwidth} 
\vspace{-20pt}
  \begin{center}
    \includegraphics[width=0.4\textwidth]{figures/learning_curve.pdf}
    \caption{Learning curve of all mappings.}
    \label{fig:app_learning_curve}
  \end{center}
\vskip -0.2in
\end{wrapfigure} 

In order to explain where the compressibility pressure comes from,
authors of \cite{nil} claim that systematic mappings are learned faster than holistic ones when a deep neural network is trained using cross-entropy loss during imitation.
They call it the ``learning speed advantage''.
Such a bias also exists (but not as strong) in more general knowledge distillation settings,
where a student network learns from a teacher's logits using a mean square error loss \cite{ren2022better}.
The origin of such a bias is the elasticity \cite{He2020elasticity} of the neural network:
the update of one $(\vx,y=k)$ pair will ``drag'' the prediction of $\vx^\dag$ to a similar direction if $\vx$ and $\vx^\dag$ are close enough in the input manifold.
As the cross-entropy loss normalizes the prediction by putting it into a simplicial space,
the increase of $p(y=k|\vx^\dag)$ will decrease other $p(y\neq k|\vx^\dag)$ significantly,
hence a stronger bias exists.

We can directly verify this hypothesis using the toy dataset mentioned before.
We create 256 datasets (each one contains 4 data samples) based on the corresponding mapping,
where $\vx$ is the concatenation of two one-hot vectors generated by the value of $\vG$.
The labels $\vy$ is just the value of $\vG$, i.e., $\mathsf{GenY}(\vG,\epsilon)=\vG$.
For each dataset,
we randomly initialize a 2-layer MLP and train it using gradient descent and a multi-task cross-entropy loss.
All the hyperparameters are the same for 256 datasets.
From the results illustrated in Figure~\ref{fig:app_learning_curve} and \ref{fig:app_learning_spd},
it is clear that the systematic mappings are learned faster than the holistic ones.
If we define the learning speed as the inverse of the integral region under the training loss and draw a histogram,
we can observe a similar pattern between learning speed and the manually designed prior in Figure~\ref{fig:app_topsim_prior}:
the compressibility pressure indeed exists for neural networks!
Such a claim could also be supported by the experimental results shown in Figure~1 in \cite{zhang2017understanding}.
In that figure,
the deep neural network learns the true label much faster than the randomly generated ones,
which matches our Figure~\ref{fig:app_learning_curve} quite well.


\begin{figure}[ht]
\vskip 0in
    \begin{center}
    \centerline{\includegraphics[width=0.9\textwidth, trim={0, 0, 0, 0}, clip]{figures/learning_speed.pdf}}
    \caption{The learning speed of all the mappings, which is quite similar to the prior in Figure~\ref{fig:app_topsim_prior}.}
    \label{fig:app_learning_spd}
    \end{center}
\vskip -0 in
\end{figure}


%\textbf{$\bullet$\quad The sample difficulty and alignment hypothesis}
\paragraph{The sample difficulty and alignment hypothesis}

Already discussed in Section~\ref{sec:toy_experiments_explanation}.
We believe that this hypothesis is easier to scale and fits the batch-based training better than the other two explanations,
as it requires the least assumptions about the model and dataset.

%\textbf{$\bullet$\quad The coding length and active basis hypothesis}
\paragraph{The coding length and active basis hypothesis}

This hypothesis is based on the analysis of a kernel ridge regression (KRR) problem and could be more theoretical (and inevitably, under more assumptions) than the other two.
Note that most of the derivations mentioned in this part could be found in \cite{mobahi2020self}.

Consider a general machine learning problem on a regression task,
in which we want to learn a mapping $f\in\mathscr{F}:\mathscr{X}\rightarrow\mathscr{Y}$ that could approximate the underlying relationship between random variables $X$ and $Y$.
As we usually have a finite number of training samples and the space of all possible mappings is large,
the model could just remember all $(\vx,y)$ pairs in the training set to achieve a perfect training performance.
To avoid this trivial solution,
we usually expect the optimal $f^*$ to have specific properties,
e.g., smoothness or Lipschitz continuousness, etc.
Hence usually,
we want to optimize a problem with a corresponding regularization term:
\begin{equation}
    f^* \triangleq \text{arg} \min_{f\in\mathscr{F}} R(f) \quad \text{s.t.} \quad \frac{1}{N}\sum_n\|f(\vx_n) - y_n \|_2^2 \leq\epsilon,
    \label{eq:app_problem_def}
\end{equation}
where $R:\mathscr{F}\rightarrow\mathbb{R}$ is regularizing $f$ and $\epsilon$ is the training loss tolerance.
The regularization term in KRR is usually the inner product of $f$ on the functional space,
i.e., $R(f)=\|f\|_\mathscr{H}$,
where $\mathscr{H}$ is a reproducing kernel Hilbert space (RKHS) determined by some kernel function $\kappa(\cdot,\cdot)$.
For example,
if we consider $\forall (x,y)\in[0,1]^2$ and $\kappa(x,y)=\min(x,y)$,
then $\|f\|_\mathscr{H}=\|f'\|_{[0,1]^2}$ \cite{scholkopf2002learning}.
In other words,
the regularizer will penalize functions with higher first-order derivatives.

In order to make the analysis generalize to other properties of $f$,
we define a linear differential operator $L$ as $[Lf]\triangleq\int_\mathscr{X} u(\vx,\cdot) f(\vx) \diff \vx$,
where $u(\cdot,\cdot)$ is a kernel function.
Then, the regularization term is:
\begin{equation}
    R(f)=\|f\|_\mathscr{H} = \langle f, f \rangle_\mathscr{H} = \langle Lf, Lf \rangle_{\mathscr{X}^2} 
        = \int_\mathscr{X}\int_\mathscr{X} u(\vx,\vx^\dag) f(\vx) f(\vx^\dag) \diff \vx \diff \vx^\dag
    \label{eq:app_regterm_def}
\end{equation}
Substituting this definition back to Equation~\ref{eq:app_problem_def} and then applying the Karush-Kuhn-Tucker (KKT) conditions,
the closed-form solution for this optimization problem is (i.e., Proposition 1 in \cite{mobahi2020self}):
\begin{equation}
    f^*(\vx) = g_{\vx}^\top (cI+G)^{-1}\vY,
\end{equation}
where $c$ is a bounded constant, $\vY=[y_1|\dots | y_N]^\top$ is the stacked training labels.
The matrix $G\in\mathbb{R}^{N\times N}$ and its vector $g_{\vx}\in\mathbb{R}^{N\times 1}$ is defined as:
\begin{equation}
    G[j,k]\triangleq\frac{1}{N} g(\vx_j, \vx_k); \quad\quad g_{\vx}[k]\triangleq\frac{1}{N} g(\vx,\vx_k).
\end{equation}
The $g(\vx,\vq)$ is the Green's function \cite{salsa2016partial} of this operator and is defined by:
\begin{equation}
    \int_\mathscr{X} u(\vx, \vx^\dag) g(\vx, \vq) \diff \vx^\dag = \delta(\vx-\vq),
\end{equation}
where $\delta$ is the Dirac delta function.
Following the definition of Green's function,
we know $G$ is positive definite and hence decompose it as:
\begin{equation}
    G = V^\top D V,
\end{equation}
where $D=\mathsf{diag}([d_1,\dots,d_N])$ is determined by its eigenvalues and $V$ contains $N$ corresponding eigenvectors.
Now, we can stack the model's prediction for different input samples $\vx_n$ and get the vector form solution of problem \ref{eq:app_problem_def}:
\begin{equation}
    \vf^* \triangleq [f^*(\vx_1) | \cdots | f^*(\vx_k)]^\top = G^\top (cI+G)^{-1}\vY = V^\top D (cI+G)^{-1}V\vY
    \label{eq:app_solution_of_f}
\end{equation}

With this solution,
following the settings in \cite{mobahi2020self},
we can explain where the compressibility pressure comes from if we only conduct the imitation phase for multiple generations.
Specifically,
the optimal model for the first generation is $\vf_0^*=V^\top D (c_0 I+G)^{-1}V\vY_0$.
Then in the following generations,
the model in generation $t$ will learn from the predictions of the model in the previous generation.
As the problem is identical (the only difference is the labels) for different generalizations,
we can have the following recursion formulas:
\begin{equation}
    \vf^*_t = V^\top D (c_tI+G)^{-1}V\vY_t \quad \text{and} \quad \vY_t=\vf^*_{t-1}.
\end{equation}
Solving this yields the expression of the labels in the $t$-th generation:
\begin{equation}
    \vY_t=V^\top A_{t-1} V \vY_{t-1} = V^\top \left(\prod_{i=0}^{t-1} A_i \right)V \vY_0,
\end{equation}
where $A_t\triangleq D(c_t I + D)^{-1}$ is a $N\times N$ diagonal matrix.
Substituting this back to Equation~\ref{eq:app_solution_of_f},
we finally obtain the following expression:
\begin{align}
    f^*_t(\vx)  &= g_{\vx}^\top V^\top D^{-1}\left(\prod_{i=0}^{t} A_i \right) V \vY_0 \\\nonumber
    \vf^*_t     &= G V^\top D^{-1} \left(\prod_{i=0}^{t} A_i \right) V \vY_0\\
                &= V^\top\left(\prod_{i=0}^{t} A_i \right) V \vY_0.
                \label{eq:app_solution_of_f_vector}
\end{align}

From this solution,
the model's prediction at $t$-th generation can be considered as a weighted combination of transformed $\vY_0$.
The matrix $V$ will first map $\vY_0$ to a space determined by the Green's function.
Different dimensions of this space are then rescaled by a diagonal matrix $\prod_{i=0}^{t} A_i$.
After that, the vector is transformed back to the origin space by multiplying $V^\top$.
Among these terms, $\prod_{i=0}^{t} A_i$ is the only one that depends on $t$.
Recall the definition of $A_t=D(c_t I+D)^{-1}$,
we can conclude that $\prod_{i=0}^{t} A_i$ is also a diagonal matrix where each entry has the form like $\prod_t\frac{d_j}{c_t+d_j}$ 
(here $d_j$ is the $j$-th eigenvalue of $G$).
As $c_t>0,\forall t$, as stated in \cite{mobahi2020self},
all the diagonal entries will gradually decrease when $t$ grows.
The dimensions with smaller $\prod_t\frac{d_j}{c_t+d_j}$ decrease faster, and vice versa.
Recall the role played by this diagonal matrix,
we can imagine that the number of active bases in $V$ is decreasing when $t$ grows,
which is a strong and unique inductive bias (i.e., compressibility pressure) introduced by this recursive training fashion\footnote{The authors in \cite{mobahi2020self} also prove that such a regularization cannot be achieved by other forms of regularizations.}.

Now, we can link these theoretical analyses to the phenomenons we observed in iterated learning.
The crux is the understanding of ``active bases''.
Consider a toy example where $\vG=[G_1, G_2]$, where each $G_i$ has 4 possible values (there are $N=16$ different objects).
Then, to memorize these 16 samples,
the model needs 16 bases like ``S 00 $\rightarrow$ blue circle''.
However, for systematic mappings, only 9 bases are enough\footnote{Specifically, we need one basis like ``S $\rightarrow$ z1 z2'', four bases like ``z0 i $\rightarrow$ some color'', and four bases like ``z1 j $\rightarrow$ some shape''. Please refer to Table~\ref{tab:app_coding_length}.}.
Finally, a degenerate mapping only needs 1 basis,
like ``S 00 $\rightarrow$ everything''.
In summary, when $t$ is large,
there is no preference for systematic mappings because the number of active bases is large enough to remember most of the training samples.
As $t$ increases,
the model then needs to be clever enough to reuse some bases,
where the structure of the mapping emerges.
If $t$ is too large,
where the compressibility pressure is too strong,
the model will degenerate into a very naive solution,
as illustrated in the third panel Figure~\ref{fig:app_ratio_language}.
Hence the expressivity pressure should be incorporated into iterated learning to avoid mode collapses,
which explains why we also need the interaction phase.


==> section_app3.tex <==
\section{Experimental Settings and More Results on Vision Datasets}
\label{sec:app_more_experiments_toy}

\subsection{Experimental Settings}
\label{sec:app_more_experiments_toy_setting}

\begin{figure}[ht]
    \begin{center}
    \centerline{\includegraphics[width=\columnwidth,trim=0 0 0 0, clip]{figures/dataset.pdf}}
    \caption{The toy vision datasets and a train/test split example. All images have size 64*64.
             Pixels in dSprite are binary values while those in 3dShape and MPI3D contain 3 channels.}
    \label{fig:dataset}
    \end{center}
\vskip -0.3in
\end{figure}

\begin{table}[ht]
\centering
\caption{Vision datasets considered in this paper.
        The numbers in the parentheses represent how many different values of the attribute.
        The last column means how many different samples we select for each $\vG$. 
        Hence the number of samples in both training and test sets of these three datasets would be 9000, 8000, and 7200.}
         \vskip 0.1in
\resizebox{1\textwidth}{!}{
\begin{tabular}{cccccccc}
\hline
         & $G_1$            & $G_2$            & $G_3$                                                                  & $G_4$                                                                & $|\mathcal{G}|$ & $\vO$                                                                        & \# per $\vG$ \\ \hline
\rowcolor[HTML]{EFEFEF} 
dSprites & shape (3)        & scale (6)        & pos-x (10 out of 32)                                                   & pos-y (10 out of 32)                                                 & 1600            & orientation (40)                                                             & 5            \\
3dShape  & floor hue (10)   & wall hue (10)    & object hue (10)                                                        & object scale (8)                                                     & 8000            & \begin{tabular}[c]{@{}c@{}}object shape (4)\\ orientation (15)\end{tabular}  & 1            \\
\rowcolor[HTML]{EFEFEF} 
MPI3D    & object color (6) & object shape (6) & \begin{tabular}[c]{@{}c@{}}horizontal x \\ (10 out of 40)\end{tabular} & \begin{tabular}[c]{@{}c@{}}vertical y\\  (10 out of 40)\end{tabular} & 3600            & \begin{tabular}[c]{@{}c@{}}size (2) camera (3)\\ background (3)\end{tabular} & 2            \\ \hline
\end{tabular}
    }
\label{tab:app_vision_datasetting}
\end{table}


%\textbf{$\bullet$\quad Data generating factors:}
\paragraph{Data generating factors}
In this paper,
we conduct experiments on three vision datasets,
i.e., dSprites~\cite{dsprites17}, 3dShapes~\cite{3dshapes18}, MPI3D-real~\cite{mpi3d},
where the ground truth $\vG$ are given.
The summary and examples of these datasets are provided in Table~\ref{tab:app_vision_datasetting} and Figure~\ref{fig:dataset}.

Here we specify how to split the dataset and generate the downstream labels using 3dShapes as an example.
We denote the hue of the floor, wall, and object as $G_1, G_2,$ and $G_3$, respectively;
each has 10 possible values,
linearly spaced in $[0,1]$.
The object scale, $G_4$,
has 8 possible values
linearly spaced in $[0,1]$.
The remaining two factors,
object shape (4 possible values) and object orientation (15 possible values),
are treated as \textit{other factors} and merged into $\vO$.
Data augmentation methods such as
adding Gaussian noise, random flipping, and so on,
are also merged into $\vO$.
Under this setting,
the universe of $\vG$, i.e., $\mathcal{G}$,
has 8000 different values,
which is further divided into $\mathcal{G}_{train}$ and $\mathcal{G}_{test}$.
For the sys-gen problem,
we assume $\mathcal{G}_{train}\cap\mathcal{G}_{test}=\emptyset$.
One measure of the difficulty of the problem is the split ratio, $\alpha=|\mathcal{G}_{train}|/|\mathcal{G}|$;
smaller $\alpha$ generally means a more challenging problem.

%\textbf{$\bullet$\quad Data generating mechanisms:}
\paragraph{Data generating mechanisms}
For the training set,
we first select $\vG\in\mathcal{G}_{train}$,
and then generate multiple
input signals using $\vx=\mathsf{GenX}(\vG,\vO)$, 
where $\vO$ is uniformly random.
The $\vx$ in the test set is generated in a similar way,
but without including data augmentation in $\vO$.
Labels for all pairs in the dataset are generated by $\vy=\mathsf{GenY}(\vG,\epsilon)$.
The main downstream task we study here is regression:
$\mathsf{GenY}(\vG,\epsilon)=\va^\top\vG+\epsilon$,
where $\va=[a_1,...,a_L]^\top$ is a column vector and all $a_i$ are chosen from $[0,1]$\footnote{We also tried a simple non-linear mapping from $\vG$ to $y$,
i.e., $\mathsf{GenY}(\vG,\epsilon)=a_1\cdot G_1  + a_2\cdot G_2 + a_3 \cdot G_4 G_3+\epsilon$,
and a multi-task scenario, where $\va\in\mathbb{R}^{|y|\times L}$ is a matrix.
The resulting trends in these settings are quite similar.}.
These examples assume $\vy$ is generated by a simple combination of different $G_i$,
where recovering the generating factors is necessary to generalize well systematically.

%\textbf{$\bullet$\quad Model and training settings:}
\paragraph{Model and training settings}
The model structure for this section is illustrated in Figure~\ref{fig:sem}.
We consider using a randomly initialized 4-layer CNN for dSprites and ReNet18 \citep{resnet} for 3dShapes and MPI3D.
% As the width of the output $\vh$ is 512,
% we embed $\vh$ to $[z_1;...;z_L]$ by multiplying a matrix $\vW_{up}\in\mathbb{R}^{512\times L'\cdot V'}$,
% where $L'$ and $V'$ are our guesses of how many generating factors and how many values they can choose from.
Unless otherwise specified,
we consider a linear head $g(\vz)$,
and a typical $\mathcal{L}_{ds}$,
i.e., cross-entropy loss for classification and mean square error loss for regression.
The networks are optimized using a standard SGD optimizer with a learning rate of $10^{-3}$ and a weight decay rate of $5*10^{-4}$.
Actually, we find the results are insensitive to these settings.


\subsection{More Results}
\label{sec:app_more_experiments_toy_results}

% \textbf{$\bullet$\quad Some interesting observations:}
\subsubsection{Some interesting observations}

\begin{figure}[ht]
     \centering
     \begin{subfigure}{0.49\textwidth}
         \centering
         \includegraphics[width=\columnwidth, trim=0 0 0 0, clip]{figures/sample_vs_argmax.pdf}
         %\caption{$y=x$}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.49\columnwidth}
         \centering
         \includegraphics[width=\columnwidth, trim=45 0 45 0, clip] {figures/entropy_change.pdf}
         %\caption{$y=3\sin x$}
     \end{subfigure}
        \caption{Left to right: 1.) zoom in on the curves of training and test loss;
                2.) demonstration of what will happen to test loss when replacing the sampling by argmax in the imitation phase;
                3.) how the average predicting entropy, i.e., $\mathbb{E}[H(\bar{z}_l)]$, changes;
                4.) histograms of predicting probabilities in different generations.
                All panels come from experiments of SEM-IL on 3dShapes.}
        \label{fig:app_sample_entropy}
\end{figure}

See the first panel in Figure~\ref{fig:app_sample_entropy},
which demonstrates the training and testing loss when training a model using SEM-IL.
In the first generation,
we see the training loss is always smaller than the test one.
The test loss then plateaus after some epochs, 
which matches our expectations.
However, in the following generations,
the test loss would decrease faster than the training one at the beginning of the interaction phase,
which is quite counter-intuitive.
We would explore why this happens and whether it is a sign of increased topological similarity in the future.

Another observation is about the sampling mechanism applied in the imitation phase.
Remember in Algorithm~\ref{alg:il},
the pseudo labels used in the imitation phase are sampled from the teacher's prediction $\bar{z}_l$.
Hence if the teacher is confident in some attributes,
the generated labels would be consistent in different epochs, and vice versa.
From Figure~\ref{fig:toy_learning_path},
we provide the scatter plot of the correlation between the teacher's confidence and the student's learning speed.
Here we verify this hypothesis through an ablation study.
Specifically,
we replace the sampling procedure with an $\mathsf{argmax}$ function,
i.e., the teacher always provides the label with the largest predicting probability regardless of its confidence.
As illustrated in the second panel in Figure~\ref{fig:app_sample_entropy},
the test performance of the $\mathsf{argmax}$-case is much worse than the standard SEM-IL method.

The benefits introduced by sampling pseudo labels can also be interpreted as we are making self-adapting $\tau$ for different input samples in SEM.
In the origin SEM,
we only have one $\tau$ to control the average entropy of the backbone's prediction (lower $\tau$ leads to peakier predicting distributions, and vice versa).
However, a model trained using SEM-IL equivalently has different $\tau$ for different $\vx$.
To understand this,
we can compare the entropy of $h_1(\vx)$ and $h_1(\vx')$,
where the teacher is confident in $(\vx, \vg_1=0)$ and less confident in $(\vx', \vg_1=0)$.
Then during imitation,
the student will remember $(\vx, \vg_1=0)$ much faster than $(\vx', \vg_1=0)$ and hence assign $\bar{z}_1=0$ higher probability when the input is $\vx$.
On the contrary,
for the input $\vx'$,
as the student might receive different corresponding pseudo labels during imitation,
it would assign a lower probability for $\bar{z}_1=0$ given $\vx'$.
As a result,
the entropy $H(\bar{z}_1 \mid \vx)$ and $H(\bar{z}_1 \mid \vx')$ of the student model would be very different as the teacher have different confidence when generating the pseudo labels,
which is equivalent as automatically selecting different $\tau$ for $\vx$ and $\vx'$.

The last two panels in Figure~\ref{fig:app_sample_entropy} demonstrate how the entropy of the model's prediction on $\vG$ changes in different generations.
(Remember the output of the backbone after SEM, i.e., $\vz=[\bar{z}_1, \dots, \bar{z}_L]$, are $L$ simplicial vectors.)
From the figures,
we see the entropy gradually decreases as the training goes on,
which means the model is becoming more and more confident in its predictions on average.
However, the last panel shows that there are still many unconfident predictions even after converging on the downstream task performance:
we speculate that these factors contain little information on $\vG$ as they might have high entropy.

% \textbf{$\bullet$\quad Influence of task difficulty:}
\subsubsection{Influence of task difficulty}

As the ground-truth generating factors are accessible for these vision datasets,
we could explore how the difficulty of the task, i.e., $\alpha$,
influence the performance gap among different methods.
As shown in Table~\ref{tab:app_alpha_3dshapes},
SEM-IL brings a significant enhancement when $\alpha$ is not too big nor too small.
When $\alpha$ is big,
the test loss might be very small and there is no room to make considerable improvement.
On another extreme,
if $\alpha$ is too small,
some attributes might be never observed during training,
which is hard for the model to extract correct generating factors.
Remember we expect to generalize to ``red circle'' by knowing the concept of red and circle from other combinations:
if there is only ``blue'' and ``box'' in the training set,
it is impractical for a model to learn such a concept (maybe the model can extrapolate, but that is another topic).
We speculate most real tasks are in a relatively small $\alpha$ regime,
as the generating factors and their possible values can be very large.
Please note that as the train/test split and $\mathsf{GenY}$ all depend on the random seeds,
the variance of the numbers in these tables could be large.
However, we observe the SEM-IL consistently outperforms other methods under each task generated by different random seeds.


\begin{table}[ht]
\centering
\caption{Relative improvement comparison for different $\alpha$ on three datasets.
         We report the average and standard error of 4 different runs.
         $\Delta_1$ is calculated by $\frac{\text{SEMIL-Baseline}}{\text{Baseline}}$,
         while $\Delta_2$ is calculated by $\frac{\text{SEMIL-Baseline}}{\text{SEMIL}}$.
         The test MSE for different settings are the numbers multiplying $10^{-3}$.
         Note that the numbers of different datasets are not comparable,
         as the model structure and generating factors of them are different.
         When $\alpha$ is too small, the model fails to converge on MPI3D, 
         which means MPI3D might be a more challenging dataset.
         }
         \vskip 0.1in
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccc}
\hline
                          & $\alpha$            & 0.8                      & 0.5                      & 0.2                      & 0.1                      & 0.02                     \\ \hline
\multirow{6}{*}{3dShapes} & Baseline            & 3.778$\pm$0.792          & 7.902$\pm$2.000          & 28.01$\pm$11.75          & 57.87$\pm$9.852          & 355.5$\pm$136.0          \\
                          & NIL-only            & 3.866$\pm$0.733          & 7.536$\pm$1.966          & 33.18$\pm$15.16          & 56.46$\pm$12.54          & 330.5$\pm$183.1          \\
                          & SEM-only            & 2.531$\pm$0.742          & 5.15$\pm$0.415           & 21.41$\pm$5.274          & 55.48$\pm$15.76          & 292.7$\pm$148.0          \\
                          & SEM-IL              & \textbf{0.633$\pm$0.117} & \textbf{1.27$\pm$0.112}  & \textbf{5.165$\pm$0.697} & \textbf{17.52$\pm$3.103} & \textbf{221.0$\pm$122.5} \\ \cline{2-7} 
                          & Relative $\Delta_1$ & 0.8324                   & \textbf{0.8396}          & 0.8156                   & 0.6972                   & 0.3783                   \\
                          & Relative $\Delta_2$ & 4.968                    & \textbf{5.236}           & 4.423                    & 2.303                    & 0.6086                   \\ \hline
\multirow{6}{*}{MPI3D}    & Baseline            & 45.42$\pm$10.97          & 61.95$\pm$17.80          & 125.9$\pm$29.30          & 234.0$\pm$34.94          & Not Converge             \\
                          & NIL-only            & 43.38$\pm$14.03          & 57.34$\pm$17.35          & 110.8$\pm$36.06          & 203.3$\pm$73.62          & Not Converge             \\
                          & SEM-only            & 42.91$\pm$10.05          & 57.69$\pm$18.34          & 116.5$\pm$38.50          & 204.1$\pm$72.68          & Not Converge             \\
                          & SEM-IL              & \textbf{31.20$\pm$8.053} & \textbf{40.33$\pm$12.12} & \textbf{73.43$\pm$22.63} & \textbf{137.8$\pm$67.36} & Not Converge             \\ \cline{2-7} 
                          & Relative $\Delta_1$ & 0.313                    & 0.349                    & \textbf{0.417}           & 0.411                    & -                        \\
                          & Relative $\Delta_2$ & 0.456                    & 0.536                    & \textbf{0.714}           & 0.698                    & -                        \\ \hline
\multirow{6}{*}{dSprites} & Baseline            & 0.172$\pm$0.145          & 7.906$\pm$2.309          & 109.2$\pm$10.28          & 313.5$\pm$28.47          & 839.7$\pm$73.85          \\
                          & NIL-only            & 0.136$\pm$0.123          & 3.678$\pm$0.869          & 56.42$\pm$7.169          & 241.0$\pm$24.68          & 630.2$\pm$32.53          \\
                          & SEM-only            & 0.126$\pm$0.119          & 7.667$\pm$1.937          & 108.8$\pm$8.563          & 315.2$\pm$23.77          & 658.0$\pm$82.52          \\
                          & SEM-IL              & \textbf{0.085$\pm$0.042} & \textbf{2.487$\pm$0.874} & \textbf{40.11$\pm$9.726} & \textbf{213.1$\pm$38.11} & \textbf{596.8$\pm$41.94} \\ \cline{2-7} 
                          & Relative $\Delta_1$ & 0.506                    & \textbf{0.685}           & 0.633                    & 0.320                    & 0.289                    \\
                          & Relative $\Delta_2$ & 1.023                    & \textbf{2.179}           & 1.722                    & 0.471                    & 0.407                    \\ \hline
\end{tabular}
    }
\label{tab:app_alpha_3dshapes}
\end{table}


% \textbf{$\bullet$\quad Other baselines from disentanglement representation learning:}
\subsubsection{Other baselines from disentanglement representation learning}
\label{app:vision:disentanglement}

Most related works consider sys-gen as an NLP or emergent language problem rather than a general representation learning problem,
so to the best of our knowledge, there are no specific advanced baselines for this concrete problem.
The most related works are some VAE-based methods in disentanglement learning.
In this part,
we re-implement $\beta$-VAE and compare them with the baseline method in our setting.
Specifically,
we first pre-train the encoder of VAE on the same training set
and then attach a task head for the downstream task to the ``$\mu$-part'' of the encoder's prediction 
(note that the encoder will output ``$\mu$-part'' and ``$\sigma$-part'' together).
We observe that the VAE-based method performs worse than the baseline method,
even though they seem to recover some disentangled factors when conducting latent traversal.
This observation is consistent with the findings in \cite{schott2022visual} and \cite{xu2022compositional},
where the authors claim that the disentangled representations are incapable of reliably generalizing to new conceptual combinations.
We also speculate that the challenging requirement of the sys-gen problem,
i.e.,  $\mathcal{G}_{train}\cap\mathcal{G}_{test}=\emptyset$,
exacerbates this:
there will not be enough variations in $\vx$ to make the VAE model capture the latent vectors precisely.
However, as VAE is also an encoder-decoder system,
it is possible to combine SEM-IL with it,
which is left for our future work.



==> section_app4.tex <==
\section{Experimental Settings and More Results on Molecular Graph Dataset}
\label{sec:app_more_experiments_real}

\begin{figure}[h]
    \begin{center}
    \centerline{\includegraphics[width=\columnwidth,trim=0 0 0 0, clip]{figures/scaffold_split.pdf}}
    \caption{Left: an example of the scaffold split, the figures are copied from \cite{wu2018moleculenet}. 
             Right: the procedure of a more challenging few-shot split used in Table~\ref{tab:main01}.}
    \label{fig:app_scaffold}
    \end{center}
\vskip -0.3in
\end{figure}

In this part,
we provide an overview of the molecular graph learning dataset we used in this paper.
\texttt{Ogbg-molhiv} and \texttt{ogbg-molpcba} \citep{ogb} are molecular property prediction datasets proposed by MoleculeNet and then adopted by open graph benchmark (OGB) project \citep{wu2018moleculenet}.
The \texttt{molhiv} dataset contains roughly 40K samples,
and the task is to predict whether a molecule is capable of inhibiting HIV replication (i.e., a binary classification task).
The \texttt{molpcba} dataset is more complex,
as it contains roughly 400K samples,
and the target is to predict 128 different bioassays,
which is a multi-task binary classification task.
\texttt{Ogb-PCQM4Mv2} \cite{pcqm} is a large-scale molecular dataset that contains roughly 4000K samples.
The task is to predict the HOMO-LUMO gap (i.e., a regression task),
which is a quantum physical property that is hard to calculate in traditional methods.
As the test split is private,
we treat the original validation split as the test split and only report the performance on it in the paper.
All of the aforementioned datasets use scaffold splitting,
which separates structurally different molecules into different subsets,
as illustrated in the left panel in Figure~\ref{fig:app_scaffold}.
Under such a split,
some specific structures in the test set might never occur during training,
which makes it a good testbed for systematic generalization ability.

To make the task more challenging,
which could simulate the scenario where $\mathsf{supp}[P_{train}(\vG)]\cap\mathsf{supp}[P_{test}(\vG)]=\emptyset$,
we prune the training set following a procedure demonstrated in the right panel of Figure~\ref{fig:app_scaffold}.
Specifically,
we first calculate the fingerprint of each $\vx$ in both training, validation, and test sets using RDKit (please refer to Section~\ref{sec:exp_real_prob} for more details).
Similar to the settings used in Table~\ref{tab:main02},
the fingerprint of each $\vx$ is defined as $\mathsf{FP}(\vx)\in\{0,1\}^{k}$.
In this vector,
$\mathsf{FP}_i(\vx)=1$ means the molecule contain the $i$-th structure.
Then, the score for each $\vx$ in the training set is defined as how many samples in the validation and test sets share the identical $\mathsf{FP}(\vx)$ with it.
To prune the training samples which are similar to the validation and test set,
we delete $\eta\%$ samples with the highest scores (for Table~\ref{tab:main01}, $\eta=50$).
If we believe these 10 structures are part of $\vG$,
the remaining training samples are more likely to have non-overlapping $\vG$ compared with the test set,
which makes the task a better testbed for systematic generalization.

The implementation of the GCN/GIN backbone used in this work is taken from the open-source code released by OGB \cite{ogb}.
We use the default setting of hyperparameters for all experiments (including baseline, baseline+, and interaction phase of SEM-only and SEM-IL).
For the backbone structure,
the depth of the GCN/GIN is 5, 
hidden embedding is 300, 
the pooling method is taking the mean, etc.
For the training on downstream tasks,
we use the AdamW \cite{loshchilov2018decoupled} optimizer with a learning rate of $10^{-3}$,
and use a cosine decay scheduler to stable the training.
For the SEM layer,
we search $L$ from $[10,200]$ and $V$ from $[5,100]$ on the validation set.
For the IL-related methods,
we select the imitation steps from \{1,000; 5,000; 10,000; 50,000; 100,000\}.
%\footnote{With batch size 64, 10,000 steps is roughly 16 epochs for \texttt{molhiv} and 2 epochs in \texttt{molpcba}.}.



